MAFIA: Multi-Adapter Fused Inclusive LanguAge Models

Pretrained Language Models (PLMs) are widely used in NLP for various tasks. Recent studies have identified various biases that such models exhibit and have proposed methods to correct these biases. However, most of the works address a limited set of bias dimensions independently such as gender, race, or religion. Moreover, the methods typically involve finetuning the full model to maintain the performance on the downstream task. In this work, we aim to modularly debias a pretrained language model across multiple dimensions. Previous works extensively explored debiasing PLMs using limited US-centric counterfactual data augmentation (CDA). We use structured knowledge and a large generative model to build a diverse CDA across multiple bias dimensions in a semi-automated way. We highlight how existing debiasing methods do not consider interactions between multiple societal biases and propose a debiasing model that exploits the synergy amongst various societal biases and enables multi-bias debiasing simultaneously. An extensive evaluation on multiple tasks and languages demonstrates the efficacy of our approach.

==> tables_ashutosh/ablation_mbert.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{lcccccc}
\toprule

\multirow{2}{*}{Model} & \multicolumn{1}{c}{STS-B} & \multicolumn{4}{c}{Bias-STS-B} & Useful fairness \\
\cmidrule(lr){2-2}
\cmidrule(lr){3-6}
\cmidrule(lr){7-7}
 & Pearson & $\delgnd$ & $\delrac$ & $\delrel$ & $\delavg$ & $\ovravg$ \\
\midrule
mBERT & {\cellcolor[HTML]{84BB9F}} \color[HTML]{000000} 0.80 & 0.12 & 0.20 & 0.22 & 0.18 & {\cellcolor[HTML]{9BD2AB}} \color[HTML]{000000} 0.66 \\
\midrule
gender (gen) & {\cellcolor[HTML]{D28092}} \color[HTML]{000000} 0.25 & {\cellcolor[HTML]{D6FFDC}} 0.06 & {\cellcolor[HTML]{D6FFDC}} 0.05 & {\cellcolor[HTML]{D6FFDC}} 0.06 & {\cellcolor[HTML]{D6FFDC}} 0.06 & {\cellcolor[HTML]{D28092}} \color[HTML]{000000} 0.24 \\
race (rac) & {\cellcolor[HTML]{FFFAD6}} \color[HTML]{000000} 0.52 & 0.28 & {\cellcolor[HTML]{D6FFDC}} 0.14 & {\cellcolor[HTML]{D6FFDC}} 0.14 & 0.18 & {\cellcolor[HTML]{FEEBC1}} \color[HTML]{000000} 0.42 \\
religion (rel) & {\cellcolor[HTML]{FFF9D4}} \color[HTML]{000000} 0.51 & 0.21 & {\cellcolor[HTML]{D6FFDC}} 0.17 & {\cellcolor[HTML]{D6FFDC}} 0.16 & {\cellcolor[HTML]{D6FFDC}} 0.18 & {\cellcolor[HTML]{FEEAC0}} \color[HTML]{000000} 0.42 \\
profession (pro) & {\cellcolor[HTML]{FABAA3}} \color[HTML]{000000} 0.37 & {\cellcolor[HTML]{D6FFDC}} 0.07 & {\cellcolor[HTML]{D6FFDC}} 0.07 & {\cellcolor[HTML]{D6FFDC}} 0.07 & {\cellcolor[HTML]{D6FFDC}} 0.07 & {\cellcolor[HTML]{FBBEA5}} \color[HTML]{000000} 0.35 \\
\midrule
gen + rac & {\cellcolor[HTML]{80B39B}} \color[HTML]{000000} 0.82 & 0.27 & 0.33 & 0.23 & 0.28 & {\cellcolor[HTML]{C8E7B3}} \color[HTML]{000000} 0.59 \\
gen + rel & {\cellcolor[HTML]{84BC9F}} \color[HTML]{000000} 0.80 & 0.14 & {\cellcolor[HTML]{D6FFDC}} 0.12 & {\cellcolor[HTML]{D6FFDC}} 0.09 & {\cellcolor[HTML]{D6FFDC}} 0.12 & {\cellcolor[HTML]{84BC9F}} \color[HTML]{000000} 0.71 \\
gen + pro & {\cellcolor[HTML]{88C3A3}} \color[HTML]{000000} 0.78 & {\cellcolor[HTML]{D6FFDC}} 0.09 & {\cellcolor[HTML]{D6FFDC}} 0.08 & {\cellcolor[HTML]{D6FFDC}} 0.05 & {\cellcolor[HTML]{D6FFDC}} 0.08 & {\cellcolor[HTML]{80B39B}} \color[HTML]{000000} 0.73 \\
rac + rel & {\cellcolor[HTML]{84BB9F}} \color[HTML]{000000} 0.80 & 0.32 & 0.39 & 0.44 & 0.38 & {\cellcolor[HTML]{F9FCD6}} \color[HTML]{000000} 0.50 \\
rac + pro & {\cellcolor[HTML]{8BC8A6}} \color[HTML]{000000} 0.77 & {\cellcolor[HTML]{D6FFDC}} 0.09 & {\cellcolor[HTML]{D6FFDC}} 0.06 & {\cellcolor[HTML]{D6FFDC}} 0.07 & {\cellcolor[HTML]{D6FFDC}} 0.07 & {\cellcolor[HTML]{82B89D}} \color[HTML]{000000} 0.72 \\
rel + pro & {\cellcolor[HTML]{83B99E}} \color[HTML]{000000} 0.81 & 0.27 & 0.21 & {\cellcolor[HTML]{D6FFDC}} 0.21 & 0.23 & {\cellcolor[HTML]{B4DFB1}} \color[HTML]{000000} 0.62 \\
\midrule
gen + rac + rel & {\cellcolor[HTML]{87C2A3}} \color[HTML]{000000} 0.79 & 0.13 & {\cellcolor[HTML]{D6FFDC}} 0.10 & {\cellcolor[HTML]{D6FFDC}} 0.07 & {\cellcolor[HTML]{D6FFDC}} 0.10 & {\cellcolor[HTML]{84BB9F}} \color[HTML]{000000} 0.71 \\
gen + rac + pro & {\cellcolor[HTML]{87C1A2}} \color[HTML]{000000} 0.79 & {\cellcolor[HTML]{D6FFDC}} 0.12 & {\cellcolor[HTML]{D6FFDC}} 0.07 & {\cellcolor[HTML]{D6FFDC}} 0.05 & {\cellcolor[HTML]{D6FFDC}} 0.08 & {\cellcolor[HTML]{80B49B}} \color[HTML]{000000} 0.72 \\
gen + rel + pro & {\cellcolor[HTML]{84BB9F}} \color[HTML]{000000} 0.80 & 0.23 & 0.35 & 0.30 & 0.29 & {\cellcolor[HTML]{D8EEB8}} \color[HTML]{000000} 0.57 \\
rac + rel + pro & {\cellcolor[HTML]{86BFA1}} \color[HTML]{000000} 0.80 & 0.21 & 0.36 & 0.32 & 0.30 & {\cellcolor[HTML]{DCF0BB}} \color[HTML]{000000} 0.56 \\
\midrule
gen + rac + rel + pro & {\cellcolor[HTML]{89C5A4}} \color[HTML]{000000} 0.78 & {\cellcolor[HTML]{D6FFDC}} 0.09 & {\cellcolor[HTML]{D6FFDC}} 0.09 & {\cellcolor[HTML]{D6FFDC}} 0.08 & {\cellcolor[HTML]{D6FFDC}} 0.09 & {\cellcolor[HTML]{83B99E}} \color[HTML]{000000} 0.71 \\
\bottomrule
\end{tabular}
    \caption{Caption}
    \label{tab:ablation_mbert}
\end{table*}
